BAGEL: Bootstrapping Agents by Guiding Exploration with Language

Following natural language instructions by executing actions in digital environments (e.g. web-browsers and REST APIs) is a challenging task for language model (LM) agents. Unfortunately, LM agents often fail to generalize to new environments without human demonstrations. This work presents BAGEL, a method for bootstrapping LM agents without human supervision. BAGEL converts a seed set of randomly explored trajectories or synthetic instructions, into demonstrations, via round-trips between two noisy LM components: an LM labeler which converts a trajectory into a synthetic instruction, and a zero-shot LM agent which maps the synthetic instruction into a refined trajectory. By performing these round-trips iteratively, BAGEL quickly converts the initial distribution of trajectories towards those that are well-described by natural language. We use BAGEL demonstrations to adapt a zero shot LM agent at test time via in-context learning over retrieved demonstrations, and find improvements of over 2-13% absolute on ToolQA and MiniWob++, with up to 13x reduction in execution failures.

==> figs/bar_plot_action_combined_backup.tex <==
\begin{figure}[htp]
\centering
\begin{subfigure}[b]{0.4\linewidth} 
\centering
\begin{tikzpicture}
    \begin{axis}[
        width=1.0\linewidth,
        height=4.0cm,
        ybar,
        ymin=0,
        ymax=60,
        xmin=-1,
        xmax=5,
        bar width=2.0mm,
        ylabel=\# Demonstrations,
        xtick=data,
        font=\small,
        xticklabel style={font=\fontsize{6}{8}\selectfont,xshift=-0.5ex,yshift=0.5ex,anchor=west,rotate=315},
        xticklabels={
Star,
Reply,
Forward,
Trash,
Delete,
        },
        yticklabel style={font=\fontsize{8}{10}\selectfont},
        ytick={0,10, 20, 30, 40},
        axis lines={left},
        axis line style={-{}},
        ]
            	
        \addplot[fill=g-yellow] coordinates {
(0, 52)
(1, 40)
(2, 19)
(3, 4)
(4, 4)
        };
\end{axis}
\end{tikzpicture}

\end{subfigure}\hfill
\begin{subfigure}[b]{0.6\linewidth} 
\centering
\begin{tikzpicture}
    \begin{axis}[
        width=1.0\linewidth,
        height=4.0cm,
        ybar,
        ymin=0,
        ymax=50,
        xmin=-1,
        xmax=9,
        bar width=2.0mm,
        ylabel=\# Demonstrations,
        xtick=data,
        font=\small,
        xticklabel style={font=\fontsize{6}{8}\selectfont,xshift=-0.5ex,yshift=0.5ex,anchor=west,rotate=315},
        xticklabels={
More,
Like,
Retweet,
Reply,
Copy,
Follow,
Mute,
Share,
Embed,
Block,
        },
        yticklabel style={font=\fontsize{8}{10}\selectfont},
        ytick={0,10, 20, 30, 40},
        axis lines={left},
        axis line style={-{}},
        ]
            	
        \addplot[fill=g-yellow] coordinates {
(0, 10)
(1, 5)
(2, 5)
(3, 4)
(4, 3)
(5, 2)
(6, 2)
(7, 2)
(8, 1)
(9, 1)
        };
\end{axis}
\end{tikzpicture}
\end{subfigure}\vspace{2pt}
\begin{subfigure}[b]{0.9\linewidth} 
\centering
\begin{tikzpicture}
    \begin{axis}[
        width=1.0\linewidth,
        height=4.0cm,
        ybar,
        ymin=0,
        ymax=50,
        xmin=-1,
        xmax=11,
        bar width=2.0mm,
        ylabel=\# Demonstrations,
        xtick=data,
        font=\small,
        xticklabel style={font=\fontsize{6}{8}\selectfont,xshift=-0.5ex,yshift=0.5ex,anchor=west,rotate=315},
        xticklabels={
\{Graph\},
\{SQL\text{,} Database\},
\{Calculator\},
\{RetrieveScirex\},
\{RetrieveAgenda\},
\{Database\},
\{Python\},
\{Python\text{,} Graph\},
\{Python\text{,} RetrieveScirex\},
\{RetrieveScirex\text{,} Graph\},
        },
        yticklabel style={font=\fontsize{8}{10}\selectfont},
        ytick={0,10, 20, 30, 40},
        axis lines={left},
        axis line style={-{}},
        ]
            	
        \addplot[fill=g-yellow] coordinates {
(0, 46)
(1, 19)
(2, 17)
(3, 13)
(4, 11)
(5, 10)
(6, 6)
(7, 2)
(8, 1)
(9, 1)
        };
\end{axis}
\end{tikzpicture}
\end{subfigure} 
\caption{Distribution of demonstrations into semantic categories. While $\ours{}$ prefer certain modes, overall we find that these demonstrations cover a wide range of tools and phenomena.} 
\label{fig:diversity}
\end{figure}


==> figs/silver_annotations.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}
    \begin{axis}[
        width=0.9\linewidth,
        height=5.0cm,
        ybar,
        ymin=0,
        ymax=80,
        xmin=-1,
        xmax=3,
        bar width=8.0mm,
        ylabel=Accuracy,
        xtick=data,
        font=\small,
        xticklabel style={font=\fontsize{6}{8}\selectfont,xshift=-0.5ex,yshift=0.5ex,align=center},
        xticklabels={Zero-shot, BAGEL, BAGEL\\(with filtering)},
        yticklabel style={font=\fontsize{8}{10}\selectfont},
        ytick={0, 10, 20, 30, 40, 50, 60, 70},
        axis lines={left},
        axis line style={-{}},
        ]
            	
        \addplot[fill=g-blue] coordinates {
        (0, 46.8)
        (1, 60.5)
        (2, 68.0)
        };
\end{axis}
\end{tikzpicture}
\caption{We report performance of $\ours{}$ where synthetic demonstrations are further filtered by human annotators, and find an improvement of over 7\% points.}
\label{fig:silver_annotations}
\end{figure}
